FiT: Flexible Vision Transformer for Diffusion Model

Nature is infinitely resolution-free. In the context of this reality, existing diffusion models, such as Diffusion Transformers, often face challenges when processing image resolutions outside of their trained domain. To overcome this limitation, we present the Flexible Vision Transformer (FiT), a transformer architecture specifically designed for generating images with unrestricted resolutions and aspect ratios. Unlike traditional methods that perceive images as static-resolution grids, FiT conceptualizes images as sequences of dynamically-sized tokens. This perspective enables a flexible training strategy that effortlessly adapts to diverse aspect ratios during both training and inference phases, thus promoting resolution generalization and eliminating biases induced by image cropping. Enhanced by a meticulously adjusted network structure and the integration of training-free extrapolation techniques, FiT exhibits remarkable flexibility in resolution extrapolation generation. Comprehensive experiments demonstrate the exceptional performance of FiT across a broad range of resolutions, showcasing its effectiveness both within and beyond its training resolution distribution. Repository available at https://github.com/whlzy/FiT.

==> backup/introduction.tex <==
\section{Introduction}

% 现有的图象生成方法对于resolution过拟合了，体现在对于resolution的泛化性过于差了。我们将其归因于对positional embedding的过拟合。

% augmentation不合理，resize，crop都会带来一些离谱的结果。

% 我们的解决方案：
% 1、立足positional embedding，来解决对resolution的过拟合问题
% 2、新的训练策略。


% Transformers现在在各个领域革命deep learning。对于生成模型也不例外，最近的出现了一系列transfomer为基础的生成模型展示出了比UNet更好的的性能表现。这些模型尽管没有UNet的归纳偏执，但是具有和UNet相当的性能表现，同时具有着稳定的scaling behavior。

% DiT是 a new class of diffusion models based on transformers。
% 它在ldm的基础上，将原来的Unet改成了一个vision transformer的结构。DiT引入了AdaLN来对模型进行condition。
% DiT展示了强大的scaling behavior of transformers在diffusion model中。
% MDT和MaskDiT是一系列基于掩码建模的transformer模型。他们基于DiT引入了decoder并在训练的时候遮掩一部分的tokens。这种方法能够提升训练的效率，同时显式地增强上下文学习能力，并改进图像中语义之间的关联关系学习。

% 尽管目前的DiT,MaskDiT,MDT展示出了在固定分辨率上的巨大潜力，但是我们发现这些模型面对训练外的分辨率会出现巨大的性能下降。这种限制阻碍了transformer based diffusion模型的各种应用。

% 当前，变压器（Transformers）正在各个领域彻底革新深度学习技术。在生成模型领域，这一趋势同样显著。近期，基于变压器的生成模型陆续亮相，其性能表现超越了传统的UNet模型。尽管这些模型不具备UNet的特有归纳偏见，但它们展示出与UNet相匹敌的性能，并且表现出稳定的规模扩展行为。

% Diffusion Transformer(DiT) is a new class of diffusion models based on transformers。它在latent diffusion model (ldm) 的基础上，用Vision Transforme结构替换了原有的Unet结构，并引入了自适应层归一化（AdaLN）来对模型进行条件限定。DiT展示了transformers在扩散模型中的强大规模扩展能力。MDT和MaskSiT是一系列基于掩码建模的变压器模型。它们在DiT的基础上增加了解码器，并在训练过程中部分遮蔽tokens，从而提高训练效率。这种方法不仅显著增强了上下文学习能力，还改进了图像中语义关联的学习。

% 然而真实世界中的图像往往并不是单一分辨率。以imagenet举例，如图所示imagenet的分辨率是非常多样的。对于过去的工作，他们往往在固定分辨率上进行训练。在这篇工作中，我们发现尽管DiT、MaskDiT和MDT在固定分辨率上展现出巨大潜力，但这些模型在面对训练之外的分辨率时性能大幅下降。这一限制成为了基于变压器的扩散模型广泛应用的障碍。我们认为这一现象的主要问题是这些模型只在单一的尺寸上进行训练，从而对训练分辨率产生过拟合。
% 另一方面，不管是Unet，还是transformer架构的模型的训练，往往通过resize和crop操作将图片处理成一个固定分辨率。
% 这种操作破坏了原始图像的aspect ratio，另一方面对于一些低分辨率的图片resize到高分辨率会引入blur。
% 虽然随机裁剪是数据扩充的一种自然形式，但它可能会泄漏到生成的样本中，使用这种处理后的图片会使得模型主动学习这种blur和这种裁剪，如上图。

% 为了克服这些问题，我们提出了一个简单而有效的训练策略，称为flexible training。
% flexible training会讲所有图像encode和patchfiy成tokens。我们首先设定了transformer的最大token上限，在这里我们采用DiT原来的token数量为了公平比较。
% flexible training不会对图像进行crop，以及对低分辨率图像resize到更高的像素。它只将图像从更高的分辨率按原来的aspect ratio resize到满足我们设定的最大token数量的尺寸。由于图片会有不同的形状不同的分辨率，所以每张图片转化后的tokens数量也不相同，flexible training在这里会将tokens padding到最大tokens数从而构建一个训练batch。由于我们引入了padding tokens，我们需要将原来的self attention改成masked self attention来规避padding token对正常token的交互。最后在进行loss计算的时候，我们只会计算那些非padding的tokens。
% 在推理的时候，我们只需要设定好想要生成图片的pos Emb，我们就可以生成不同尺寸的图片。

% 另一方面，我们发现最初始的DiT对于外推不是特别有效果。从大语言模型那边获得灵感，我们去除了在vision transformer中常用的sincos绝对位置编码，而是使用RoPE2d位置编码，同时我们将DiT中的MLP换成了SwiGLU。我们的实验证明了这些改动不仅能够提升训练内分辨率的性能还能够大幅提升训练外分辨率的性能。经过修改后的FiT结构可以兼容大语言模型的一些外推技术，解决token的长度外推问题。但是直接将其应用到FiT上并不是特别work。我们针对这些技术进行了修正来适配2d的RoPE编码。经过修正后的FiT进一步在各个分辨率aspect ratio获得了性能的提升。

% 更具体来说，我们对模型分别在训练分辨率和训练外分辨率上进行了测试，还测试了不同的aspect ratio的生成效果。将上面的技术汇集到一起，最终FiT实现了优越的性能表现，无论是在训练分辨率还是在外推分辨率上。


% Transformer is revolutionizing various fields of deep learning. This trend is particularly evident in the realm of generative models. Recently, a series of transformer-based generative models have been introuduced, surpassing the performance of traditional UNet models. Although these models lack the unique inductive biases inherent in UNet, they demonstrate comparable performance to UNet and exhibit stable scalability.
Transformers are revolutionizing various fields of deep learning.
For image generation, recent advancements have seen transformer-based generative models outperforming traditional UNet-based models. 
Despite lacking the unique inductive biases of UNet, these models achieve comparable performance and exhibit stable scalability.

% Diffusion transformer (DiT) is a novel class of diffusion models based on the transformer architecture. Building upon the latent diffusion model (LDM), it replaces the original UNet structure with a vision transformer architecture and introduces adaptive layer normalization zero (AdaLN) for conditional modeling. DiT demonstrates the impressive scalability of Transformers in the domain of diffusion models. MDT and MaskDiT are part of a series of diffusion transformer models based on masked modeling. These models build upon DiT by adding a decoder and partially masking some tokens during training, thereby enhancing training efficiency. This approach not only significantly improves the learning of contextual information but also advances the learning of semantic associations in images.
% The Diffusion Transformer (DiT) represents a novel class of diffusion models. 
The Diffusion transformer (DiT), a novel class of diffusion models, epitomizes this advancement.
% Building on the Latent Diffusion Model (LDM), DiT integrates a vision transformer architecture and introduces Adaptive Layer Normalization Zero (AdaLN) for enhanced conditional modeling. 
Originating from the latent diffusion model (LDM), DiT integrates a vision transformer architecture with adaptive layer normalization zero (AdaLN) for enhanced conditional modeling.
Its scalability underscores the transformer's potential in diffusion models. 
% Masked Diffusion Transformer (MDT) and Masked Image Diffusion Transformer (MaskDiT) extend this concept through masked modeling, adding a decoder, and training with partially masked tokens to improve contextual understanding and semantic associations in images.
Subsequent developments like MDT and MaskDiT, which extend DiT with a decoder and masked modeling, further optimize training efficiency and improve contextual and semantic learning in images.

% In the real world, images often come in a variety of resolutions. Taking ImageNet as an example, it is evident that the resolution of images is highly diverse, as shown in Fig.~\ref{fig:imagenet}. Past research typically focused on training models at a fixed resolution. However, we find that while DiT, MaskDiT, and MDT show great potential at fixed resolutions, their performance significantly deteriorates when dealing with images of resolutions different from the training resolution. This limitation hampers the widespread application of Transformer-based diffusion models. We think the primary issue is that these models are trained only at a fixed resolution, leading to overfitting to the training resolution. Moreover, both Unet and transformer-based models are trained with images resized and cropped to a fixed resolution, which alters the original aspect ratio and introduces blur when processing low-resolution images. Although random cropping is a natural form of data augmentation, it can inadvertently be reflected in the generated samples, leading the model to actively learn this blur and cropping effect, as illustrated in the Fig.~\ref{}.
% However, a challenge arises when dealing with varying image resolutions, such as those in ImageNet. 
A critical challenge in real-world applications is the diversity of image resolutions, exemplified by ImageNet's varied resolution spectrum (illustrated in Fig.~\ref{fig:imagenet}). 
Traditional models, including DiT, MaskDiT, and MDT, perform optimally at fixed resolutions but falter with differing resolutions. 
% This issue, we believe, stems from their training solely on fixed-resolution images, leading to overfitting. 
% Additionally, the common practice of resizing and cropping images alters their original aspect ratio and introduces blur in low-resolution images. This effect is inadvertently learned by the model, as evidenced in generated samples.
This limitation, we believe, stems from overfitting to a specific training resolution and the alteration of the original aspect ratios due to resizing and cropping.

\input{figure/fig_imagenet}


% To address these issues, we propose a simple yet effective training strategy called "flexible training" for our flexible vision transformer. This strategy encodes and patchify images into tokens. We set a maximum token limit for the transformer, using the same as the token length of DiT for a fair comparison. Flexible training does not crop images or resize low-resolution images to higher pixels. Instead, it resizes higher-resolution images down to a size that meets our maximum token count, maintaining the original aspect ratio. Due to varying shapes and resolutions, the number of tokens per image differs; hence, flexible training involves padding tokens to the maximum count to create a training batch. With the introduction of padding tokens, we shifted from traditional self-attention to masked self-attention to prevent interactions with padding tokens. During loss computation, we only consider non-padding tokens. For inference, by setting the desired positional embeddings (pos Emb), we can generate images of varying sizes. Additionally, we observed that the original DiT was not particularly effective in extrapolation. Inspired by large language models, we replaced the commonly used sincos absolute position encoding in vision transformers with RoPE2d positional encoding and switched the MLP in DiT to SwiGLU. Our experiments demonstrate that these modifications not only enhance performance at training-internal resolutions but also significantly improve training-external resolution performance. The modified FiT structure accommodates some extrapolation techniques from large language models, addressing the issue of token length extrapolation. However, applying these techniques directly to FiT was not entirely effective. We adapted these techniques to fit the 2D RoPE encoding. The revised FiT further improved performance across various resolutions and aspect ratios.

To overcome these limitations, 
% we introduce a ``Flexible Training" strategy for our Flexible Vision Transformer (FiT). 
% we introduce a ``Flexible Training" strategy for our Flexible Vision Transformer (FiT). 
we introduce a novel Scalable \textbf{F}lexible V\textbf{i}sion \textbf{T}ransformer (FiT) for the Diffusion Model. FiT is designed for generating images with \textit{arbitrary resolutions and aspect ratios}.
To achieve this, FiT considers three aspects of modifications: \textbf{network architecture}, \textbf{training strategy}, and \textbf{inference strategy}. 

During training, FiT retains the original aspect ratio of images by resizing higher-resolution images to fit a maximum token limit,
% akin to DiT’s token length, 
without cropping or resizing low-resolution images. 
% The varying shapes and resolutions of images necessitate padding tokens for consistent batch sizes. 
% We employ masked self-attention to ignore these padding tokens and focus loss computation solely on non-padding tokens. 
To the best of our knowledge, FiT is the first work keeping various image resolutions for training. 

For inference, 

positional embeddings are adjusted to generate images of varying sizes. 
Notably, the original DiT struggled with resolution extrapolation generation. 
To address this, we integrated RoPE2d positional encoding and replaced the MLP with SwiGLU, drawing inspiration from large language models. 
These modifications enhance performance across resolutions. 
However, directly applying token length extrapolation techniques from large language models to FiT was suboptimal. 
We adapted these techniques for 2D RoPE encoding, further improving FiT’s performance across various resolutions and aspect ratios.

\todo{add experiments illustration}

Our FiT-XL/2 model trained only 1.7M steps outperforms all SOTA CNN models ("ADM-G,U", "LDM-4-G") and transformer models ("U-ViT-H/2-G, DiT-XL/2-G), surpassing it by a large margin on the resolutions of $160\times320$, $128\times384$, $320\times320$, $224\times448$, and $160\times480$.
The performance of the FiT-XL/2 model significantly improved further after the adoption of our training-free extrapolation technique.

compared to the DiT-XL

, which was trained for 7M steps, the FiT-XL lags by 2 FID score points at a resolution of 256x256. However, at other resolutions, the FiT-XL d, significantly surpassing all other models.

% Our contributions are three-fold:
% 1. We propose a simple and efficient flexible transformer training framework for diffusion model, enabling training our FiT in various aspect-ratio images without cropping.
% 2. We carefully adjust the architecture of FiT making it more suitable than DiT for generating images with different resolutions. FiT achieves superior results at different resolutions on the class-conditional ImageNet generation benchmark.
% 3. We discover that some recent training free extrapolation techniques used in LLMs, after proper modifications, can significantly improve the resolution extrapolation ability of FiT.
Our contributions are threefold:
\begin{itemize}
    \item We present a flexible transformer training framework for diffusion models, enabling efficient training of FiT on images with diverse aspect ratios without cropping.
    \item We refine FiT's architecture, making it more adept than DiT at generating images of different resolutions, as evidenced by superior results on the class-conditional ImageNet generation benchmark.
    \item We adapt training-free extrapolation techniques from large language models, significantly enhancing FiT's resolution extrapolation capabilities.
\end{itemize}

% \begin{itemize}
%     \item We propose a simple and efficient flexible transformer training framework for diffusion model, enabling training our FiT in various aspect-ratio images without cropping.
%     \item We adjust the transformer architecture of FiT making it more suitable for generating images with various resolutions. FiT achieves superior results at different resolutions on the class-conditional ImageNet generation benchmark.
%     \item We discover that some recent training free extrapolation techniques used in LLMs, after proper modifications, can significantly improve the resolution extrapolation ability of FiT.
% \end{itemize}












==> backup/introduction_2.tex <==
\section{Introduction}
% Transformer is revolutionizing various fields of deep learning. This trend is particularly evident in the realm of generative models. Recently, a series of transformer-based generative models have been introuduced, surpassing the performance of traditional UNet models. Although these models lack the unique inductive biases inherent in UNet, they demonstrate comparable performance to UNet and exhibit stable scalability.
Transformers are revolutionizing various fields of deep learning.
For image generation, recent advancements have seen transformer-based generative models outperforming traditional UNet-based models. 
Despite lacking the unique inductive biases of UNet, these models achieve comparable performance and exhibit stable scalability.

% Diffusion transformer (DiT) is a novel class of diffusion models based on the transformer architecture. Building upon the latent diffusion model (LDM), it replaces the original UNet structure with a vision transformer architecture and introduces adaptive layer normalization zero (AdaLN) for conditional modeling. DiT demonstrates the impressive scalability of Transformers in the domain of diffusion models. MDT and MaskDiT are part of a series of diffusion transformer models based on masked modeling. These models build upon DiT by adding a decoder and partially masking some tokens during training, thereby enhancing training efficiency. This approach not only significantly improves the learning of contextual information but also advances the learning of semantic associations in images.
% The Diffusion Transformer (DiT) represents a novel class of diffusion models. 
The Diffusion transformer (DiT), a novel class of diffusion models, epitomizes this advancement.
% Building on the Latent Diffusion Model (LDM), DiT integrates a vision transformer architecture and introduces Adaptive Layer Normalization Zero (AdaLN) for enhanced conditional modeling. 
Originating from the latent diffusion model (LDM), DiT integrates a vision transformer architecture with adaptive layer normalization zero (AdaLN) for enhanced conditional modeling.
Its scalability underscores the transformer's potential in diffusion models. 
% Masked Diffusion Transformer (MDT) and Masked Image Diffusion Transformer (MaskDiT) extend this concept through masked modeling, adding a decoder, and training with partially masked tokens to improve contextual understanding and semantic associations in images.
Subsequent developments like MDT and MaskDiT, which extend DiT with a decoder and masked modeling, further optimize training efficiency and improve contextual and semantic learning in images.

% In the real world, images often come in a variety of resolutions. Taking ImageNet as an example, it is evident that the resolution of images is highly diverse, as shown in Fig.~\ref{fig:imagenet}. Past research typically focused on training models at a fixed resolution. However, we find that while DiT, MaskDiT, and MDT show great potential at fixed resolutions, their performance significantly deteriorates when dealing with images of resolutions different from the training resolution. This limitation hampers the widespread application of Transformer-based diffusion models. We think the primary issue is that these models are trained only at a fixed resolution, leading to overfitting to the training resolution. Moreover, both Unet and transformer-based models are trained with images resized and cropped to a fixed resolution, which alters the original aspect ratio and introduces blur when processing low-resolution images. Although random cropping is a natural form of data augmentation, it can inadvertently be reflected in the generated samples, leading the model to actively learn this blur and cropping effect, as illustrated in the Fig.~\ref{}.
% However, a challenge arises when dealing with varying image resolutions, such as those in ImageNet. 
A critical challenge in real-world applications is the diversity of image resolutions, exemplified by ImageNet's varied resolution spectrum (illustrated in Fig.~\ref{fig:imagenet}). 
Traditional models, including DiT, MaskDiT, and MDT, perform optimally at fixed resolutions but falter with differing resolutions. 
% This issue, we believe, stems from their training solely on fixed-resolution images, leading to overfitting. 
% Additionally, the common practice of resizing and cropping images alters their original aspect ratio and introduces blur in low-resolution images. This effect is inadvertently learned by the model, as evidenced in generated samples.
This limitation, we believe, stems from overfitting to a specific training resolution and the alteration of the original aspect ratios due to resizing and cropping.

\input{figure/fig_imagenet}


% To address these issues, we propose a simple yet effective training strategy called "flexible training" for our flexible vision transformer. This strategy encodes and patchify images into tokens. We set a maximum token limit for the transformer, using the same as the token length of DiT for a fair comparison. Flexible training does not crop images or resize low-resolution images to higher pixels. Instead, it resizes higher-resolution images down to a size that meets our maximum token count, maintaining the original aspect ratio. Due to varying shapes and resolutions, the number of tokens per image differs; hence, flexible training involves padding tokens to the maximum count to create a training batch. With the introduction of padding tokens, we shifted from traditional self-attention to masked self-attention to prevent interactions with padding tokens. During loss computation, we only consider non-padding tokens. For inference, by setting the desired positional embeddings (pos Emb), we can generate images of varying sizes. Additionally, we observed that the original DiT was not particularly effective in extrapolation. Inspired by large language models, we replaced the commonly used sincos absolute position encoding in vision transformers with RoPE2d positional encoding and switched the MLP in DiT to SwiGLU. Our experiments demonstrate that these modifications not only enhance performance at training-internal resolutions but also significantly improve training-external resolution performance. The modified FiT structure accommodates some extrapolation techniques from large language models, addressing the issue of token length extrapolation. However, applying these techniques directly to FiT was not entirely effective. We adapted these techniques to fit the 2D RoPE encoding. The revised FiT further improved performance across various resolutions and aspect ratios.

To overcome these limitations, 
% we introduce a ``Flexible Training" strategy for our Flexible Vision Transformer (FiT). 
% we introduce a ``Flexible Training" strategy for our Flexible Vision Transformer (FiT). 
we introduce a novel Scalable \textbf{F}lexible V\textbf{i}sion \textbf{T}ransformer (FiT) for the Diffusion Model. FiT is designed for generating images with \textit{arbitrary resolutions and aspect ratios}.
\todo{Introduce resolution extrapolation.}
To achieve this, FiT considers three aspects of modifications: \textbf{network architecture}, \textbf{training strategy}, and \textbf{inference strategy}. 

\noindent \textbf{Network architecture.} 
FiT backbone is based on DiT. However, the original DiT struggled with resolution extrapolation generation. 
To generate images of varying sizes, the key is adjusting positional embeddings. 
Drawing inspiration from large language model advances,  
we integrated RoPE2d positional encoding and replaced the MLP of DiT with SwiGLU.

\noindent \textbf{Training strategy.} 
During training, FiT retains the original aspect ratio of images by resizing higher-resolution images to fit a maximum token limit, without cropping or resizing low-resolution images. 
To the best of our knowledge, FiT is the first work keeping various image resolutions for training. 

\noindent \textbf{Inference strategy.} 
% For inference, 
% positional embeddings are adjusted to generate images of varying sizes. 
% Notably, the original DiT struggled with resolution extrapolation generation. 
% To address this, we integrated RoPE2d positional encoding and replaced the MLP with SwiGLU, drawing inspiration from large language models. 
% These modifications enhance performance across resolutions. 
% However, directly applying token length extrapolation techniques from large language models to FiT was suboptimal. 
% We adapted these techniques for 2D RoPE encoding, further improving FiT’s performance across various resolutions and aspect ratios.
Large language models use token length extrapolation techniques to generate arbitrary lengths of texts. 
However, directly applying them to FiT was suboptimal. 
We adapted these techniques for 2D RoPE encoding, further improving FiT’s performance across various resolutions and aspect ratios.

\todo{add experiments illustration}

Our FiT-XL/2 model trained only 1.7M steps outperforms all SOTA CNN models ("ADM-G,U", "LDM-4-G") and transformer models ("U-ViT-H/2-G, DiT-XL/2-G), surpassing it by a large margin on the resolutions of $160\times320$, $128\times384$, $320\times320$, $224\times448$, and $160\times480$.
The performance of the FiT-XL/2 model significantly improved further after the adoption of our training-free extrapolation technique. compared to the DiT-XL, which was trained for 7M steps, the FiT-XL lags by 2 FID score points at a resolution of 256x256. However, at other resolutions, the FiT-XL d, significantly surpassing all other models.

% Our contributions are three-fold:
% 1. We propose a simple and efficient flexible transformer training framework for diffusion model, enabling training our FiT in various aspect-ratio images without cropping.
% 2. We carefully adjust the architecture of FiT making it more suitable than DiT for generating images with different resolutions. FiT achieves superior results at different resolutions on the class-conditional ImageNet generation benchmark.
% 3. We discover that some recent training free extrapolation techniques used in LLMs, after proper modifications, can significantly improve the resolution extrapolation ability of FiT.
Our contributions are threefold:
\begin{itemize}
    \item We present a flexible transformer training framework for diffusion models, enabling efficient training of FiT on images with diverse aspect ratios without cropping.
    \item We refine FiT's architecture, making it more adept than DiT at generating images of different resolutions, as evidenced by superior results on the class-conditional ImageNet generation benchmark.
    \item We adapt training-free extrapolation techniques from large language models, significantly enhancing FiT's resolution extrapolation capabilities.
\end{itemize}

% \begin{itemize}
%     \item We propose a simple and efficient flexible transformer training framework for diffusion model, enabling training our FiT in various aspect-ratio images without cropping.
%     \item We adjust the transformer architecture of FiT making it more suitable for generating images with various resolutions. FiT achieves superior results at different resolutions on the class-conditional ImageNet generation benchmark.
%     \item We discover that some recent training free extrapolation techniques used in LLMs, after proper modifications, can significantly improve the resolution extrapolation ability of FiT.
% \end{itemize}












==> backup/introduction_3.tex <==
\section{Introduction}
% \xihui{Why start from transformer-based diffusion? Why not start from ``current t2i models face difficulties when generalizing to arbitrary resolutions''? The current version takes three paragraphs to introduce the challenge that we try to address.}

% Transformers are significantly impacting various domains within deep learning, as evidenced by the breakthroughs achieved with large language models (LLMs).
% In image generation, transformer-based generative models are beginning to outperform traditional UNet-based architectures, despite lacking inductive biases of UNet. These models demonstrate comparable effectiveness and remarkable scalability.

% The Diffusion Transformer (DiT), a novel class of diffusion models, underscores this progress.
% Originating from the latent diffusion model (LDM), 
% DiT and U-ViT integrate a vision transformer architecture for image generation.
% Its scalability underscores the potential benefits of integrating transformer architectures into diffusion models. Further developments, such as MDT and MaskDiT, which augment DiT with a decoder and masked modeling strategy, significantly enhance training efficiency and improve contextual and semantic learning in images.

% A critical challenge in deploying these models in practical applications is their performance across a wide range of image resolutions. For instance, as illustrated in Fig.~\ref{fig:imagenet}, images span various resolution spectrums. 
Current text-to-image generation models face difficulties when generalizing to arbitrary resolutions. 
% However, current image generation models, including DiT, MDT, U-ViT, ADM and LDM, excel within specific resolution ranges but falter with images of varying resolutions. 
For example, The Diffusion Transformer (DiT)~\cite{} family, excels within specific resolution ranges but falters with images of varying resolutions. 
This limitation stems from the fact that DiT does not utilize dynamic resolution images during its training process, resulting in the model's inadequacy in handling varying token lengths or resolutions. 

% To address these limitations, 
To address the fixed resolution limitation, 
we introduce the \textbf{F}lexible V\textbf{i}sion \textbf{T}ransformer (FiT) for Diffusion Models, designed to generate images at \textit{arbitrary resolutions and aspect ratios}. 
FiT innovates through strategic enhancements in \textbf{network architecture}, \textbf{flexible training pipeline}, and \textbf{inference processes}.

\noindent \textbf{Network architecture.} 
The FiT model evolves from the DiT architecture but addresses its limitations in resolution extrapolation. 
A critical component for generating images of various sizes is the positional embedding. 
Inspired by the success of Rotary Positional Embedding (RoPE) in large language models, we incorporate 2D RoPE instead of Absolute Positional Embedding.
Furthermore, we replace DiT's Multilayer Perceptron (MLP) with Swish-Gated Linear Unit (SwiGLU), which is commonly used in recent large language models.
% We replace Multi-Head Self-Attention (MHSA) in DiT with Masked Multi-Head Self-Attention (Masked MHSA) for dealing with the padding tokens used in our flexibel training pipeline.
Moreover, we substitute DiT's Multi-Head Self-Attention (MHSA) with Masked Multi-Head Self-Attention (Masked MHSA) to handle the padding tokens introduced in our proposed flexible training pipeline.
% Flexible training pipeline introduces padding tokens for flexibly packing dynamic sequences into a batch, so we 


% and replace DiT's Multilayer Perceptron (MLP) with Swish-Gated Linear Unit (SwiGLU), Multi-Head Self-Attention (MHSA) with Masked Multi-Head Self-Attention (Masked MHSA). 
% \xihui{Too specific. Any intuitions and motivations for replacing those layers?}

\noindent \textbf{Flexible Training Pipeline.} 
FiT uniquely preserves the original aspect ratio of images by resizing higher-resolution images to fit within a maximum token limit, thus avoiding the cropping of higher-resolution images or resizing of lower-resolution images.
To the best of our knowledge, FiT is the first transformer-based generation model to maintain diverse image resolutions throughout training.

\noindent \textbf{Inference process.} 
Large language models use token length extrapolation techniques to generate arbitrary lengths of texts. 
While large language models employ token length extrapolation techniques for generating text of arbitrary lengths, a direct application of these technologies to FiT yielded suboptimal results. We tailored these techniques for 2D RoPE, thereby enhancing FiT’s performance across a spectrum of resolutions and aspect ratios.

\input{figure/fig_performance}

% Our FiT-XL/2 model trained only 1.7M steps outperforms all SOTA CNN models ("ADM-G,U", "LDM-4-G") and transformer models ("U-ViT-H/2-G, DiT-XL/2-G), surpassing it by a large margin on the resolutions of $160\times320$, $128\times384$, $320\times320$, $224\times448$, and $160\times480$.
% The performance of the FiT-XL/2 model significantly improved further after the adoption of our training-free extrapolation technique. compared to the DiT-XL, which was trained for 7M steps, the FiT-XL lags by 2 FID score points at a resolution of 256x256. However, at other resolutions, the FiT-XL d, significantly surpassing all other models.

% Our FiT-XL/2 model, after training for only 1.7 million steps, outperforms all state-of-the-art CNN ("ADM-G,U", "LDM-4-G") and transformer ("U-ViT-H/2-G, DiT-XL/2-G) models by a significant margin across resolutions of $160\times320$, $128\times384$, $320\times320$, $224\times448$, and $160\times480$. The performance of FiT-XL/2 significantly advances further with our training-free extrapolation technique. Compared to the DiT-XL, which underwent training for 7 million steps, FiT-XL lags by merely 2 FID score points at a resolution of 256x256 but significantly surpasses all competing models at other resolutions.
Our highest Gflop FiT-XL/2 model, after training for only 1.8 million steps, outperforms all state-of-the-art CNN and transformer models by a significant margin across resolutions of $160\times320$, $128\times384$, $320\times320$, $224\times448$, and $160\times480$. The performance of FiT-XL/2 significantly advances further with our training-free extrapolation technique. Compared to the DiT-XL/2 training for 7 million steps, FiT-XL/2 lags slightly at the resolution of $256\times256$ but significantly surpasses it at all other resolutions.
In summary, our contributions are threefold:
% \begin{compactitem}
%     \item Introduction of FiT, a scalable and flexible vision transformer tailored for image diffusion models, capable of generating images at any resolution and aspect ratio.
    
%     \item Implementation of innovative design features in FiT, including a unique transformer architecture for dynamic token length, a flexible training pipeline that eliminates the need for cropping, and an inference strategy optimized for arbitrary resolution generation.
    
%     \item Demonstration that the FiT-XL/2 model achieves state-of-the-art performance across a variety of resolution settings.
% \end{compactitem}
In summary, our contributions lie in the novel introduction of FiT, a scalable and flexible vision transformer tailored for image diffusion models, capable of generating images at any resolution and aspect ratio. We implement three innovative design features in FiT, including a unique transformer architecture for dynamic token length, a flexible training pipeline that eliminates the need for cropping, and an inference strategy optimized for arbitrary resolution generation. Experiments demonstrate that the FiT-XL/2 model achieves state-of-the-art performance across a variety of resolution settings. 

% \xihui{It's not common to write the contribution in this way. usually three different keypoints, or two keypoints + experiment highlight. If keep this logic, you can merge the three items into a single paragraph.}



\input{figure/fig_imagenet}

==> figure/fig_performance.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/performance.pdf}
    \caption{
        performance
    }
    \label{fig:performance}
\end{figure}

==> table/ablation_extrapolation_hard.tex <==
\begin{table*}[t]
\centering
% \addtolength{\tabcolsep}{-1pt}

\begin{adjustbox}{max width=1.\textwidth}
\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule[1.2pt]
\multirow{2}*{Method}&\multicolumn{5}{c|}{384$\times$384 (1:1)}&\multicolumn{5}{c|}{256$\times$512 (1:2)}&\multicolumn{5}{c}{192$\times$576 (1:3)} \\

& \textbf{FID$\downarrow$} & \textbf{sFID$\downarrow$} & \textbf{IS$\uparrow$} & \textbf{Prec.$\uparrow$} & \textbf{Rec.$\uparrow$}
& \textbf{FID$\downarrow$} & \textbf{sFID$\downarrow$} & \textbf{IS$\uparrow$} & \textbf{Prec.$\uparrow$} & \textbf{Rec.$\uparrow$}  
& \textbf{FID$\downarrow$} & \textbf{sFID$\downarrow$} & \textbf{IS$\uparrow$} & \textbf{Prec.$\uparrow$} & \textbf{Rec.$\uparrow$}  \\
% & \textbf{FID} & \textbf{sFID} & \textbf{IS} & \textbf{Prec.} & \textbf{Rec.}
% & \textbf{FID} & \textbf{sFID} & \textbf{IS} & \textbf{Prec.} & \textbf{Rec.}  
% & \textbf{FID} & \textbf{sFID} & \textbf{IS} & \textbf{Prec.} & \textbf{Rec.}  \\

\midrule

DiT-B & 138.93 & 153.54 & 10.36 & 0.13 & 0.21 &     
130.05 & 128.61 & 11.55 & 0.15 & 0.24 &    
184.39 & 141.90 & 7.32 & 0.053 & 0.13 \\

DiT-B + EI & 159.03 & 124.40 & 7.05 & 0.068 & 0.18 &    
148.52 & 98.38 & 9.93 & 0.088 & 0.23 &    
195.06 & 116.96 & 5.60 & 0.030 & 0.11 \\

DiT-B + PI & 160.73 & 121.30 & 7.26 & 0.065 & 0.18 &    
145.04 & 95.12 & 10.69 & 0.094 & 0.22 &    
186.11 & 117.79 & 5.74 & 0.034 & 0.14 \\
\midrule
FiT-B & 81.79 & \textbf{59.49} & 25.21 & 0.3178 & 0.4528 & 55.21 & \textbf{40.50} & 33.67 & 0.4320 & 0.4473 & \textbf{72.31} & \textbf{41.65} & 24.47 & 0.327 & 0.4231 \\

FiT-B + PI & 124.01 & 119.07 & 14.47 & 0.1386 & 0.2547 & 208.46 & 134.87 & 6.53 & 0.0304 & 0.0816 & 263.30 & 148.75 & 4.66 & 0.0136 & 0.0183 \\

FiT-B + YaRN & 63.81 & 73.76 & 39.58 & 0.3718 & 0.4365 & 136.41 & 108.40 & 23.43 & 0.1580 & 0.3062 & 171.80 & 107.93 & 17.84 & 0.1054 & 0.2387 \\

FiT-B + PartNTK & 83.30 & 79.90 & 31.22 & 0.2977 & 0.4348 & 166.91 & 109.84 & 18.28 & 0.1095 & 0.3845 & 197.02 & 107.03 & 14.49 & 0.0726 & 0.2235 \\

FiT-B + NTK & 73.36 & 57.23 & 29.23 & 0.3454 & 0.4608 & 58.47 & 47.18 & 35.48 & 0.3910 & 0.4694 & 79.25 & 47.49 & 25.07 & 0.2854 & 0.4157 \\

FiT-B + VisionYaRN & \textbf{63.81} & 73.76 & \textbf{39.58} & \textbf{0.3718} & 0.4365 & \textbf{50.15} & 63.03 & \textbf{43.48} & \textbf{0.4331} & 0.4181 & 78.59 & 70.34 & \textbf{27.85} & 0.2988 & 0.354 \\

FiT-B + VisionNTK & 73.36 & 57.24 & 29.24 & 0.3456 & \textbf{0.4613} & 55.88 & 42.80 & 34.96 & 0.4162 & \textbf{0.4605} & 73.16 & 43.03 & 25.54 & \textbf{0.3171} & \textbf{0.4319} \\

\bottomrule[1.2pt]

\end{tabular}
\end{adjustbox}

\caption{Benchmarking class-conditional image generation on ImageNet out-of-distribution resolution. (400k)}
\label{tab:in1k_ood}
\end{table*}
